Descriptive Complexity in Lean: Completeness by First-Order Reductions

We show that descriptive complexity can serve as a foundation for formalizing computational complexity results in a proof assistant, by constructing a Lean library centered around the following concepts: decision problems are isomorphism-invariant predicates on finite structures; complexity classes are defined by their logical characterization; membership is shown by definability witnesses; hardness is shown by first-order reductions from a known hard problem. We also establish bridges to traditional machine models such as (non)deterministic Turing machines. The library proves 73 completeness results, on 68 problems or problem families, over 14 different classes; relations between the classes established inside the logic and not by machine simulation, among them NL = coNL and the Abiteboul-Vianu theorem; and unconditional lower bounds, among them $\mathrm{FO}(\leq) \subsetneq \mathrm{FO}(\leq, \mathrm{TC})$ and the failure of order-free FO(IFP) to capture PTIME.

==> figures/np-reductions.tex <==

\begin{tikzpicture}[>=latex,line join=bevel,]
%%
\begin{scope}
  \pgfsetstrokecolor{black}
  \definecolor{strokecol}{rgb}{1.0,1.0,1.0};
  \pgfsetstrokecolor{strokecol}
  \definecolor{fillcol}{rgb}{1.0,1.0,1.0};
  \pgfsetfillcolor{fillcol}
  \filldraw (0.0bp,0.0bp) -- (0.0bp,382.04bp) -- (1305.0bp,382.04bp) -- (1305.0bp,0.0bp) -- cycle;
\end{scope}
  \definecolor{strokecolor}{rgb}{0.2,0.2,0.2};
  \node (ZeroOneIP) at (44.0bp,17.0bp) [draw=strokecolor,rectangle,rounded,filled,karp] {\shortstack{0-1 INTEGER\\PROGRAMMING}};
  \definecolor{strokecolor}{rgb}{0.33,0.33,0.33};
  \node (lt0) at (537.0bp,17.0bp) [draw=strokecolor,draw=none,solid,legend] {\fored{} order-free};
  \coordinate (la0) at (434.0bp,17.0bp);
  \definecolor{strokecolor}{rgb}{0.33,0.33,0.33};
  \node (lt1) at (753.0bp,17.0bp) [draw=strokecolor,draw=none,solid,legend] {\foredord{} ordered};
  \coordinate (la1) at (640.0bp,17.0bp);
  \definecolor{strokecolor}{rgb}{0.33,0.33,0.33};
  \node (lt2) at (994.0bp,17.0bp) [draw=strokecolor,draw=none,solid,legend] {\foredrel{} relativized};
  \coordinate (la2) at (866.0bp,17.0bp);
  \definecolor{strokecolor}{rgb}{0.2,0.2,0.2};
  \node (lk) at (1212.0bp,17.0bp) [draw=strokecolor,rectangle,rounded,filled,karp,legend] {one of Karp's 21};
  \definecolor{strokecolor}{rgb}{0.33,0.33,0.33};
  \node (ESO) at (794.0bp,370.02bp) [draw=strokecolor,ellipse,rounded,filled] {∃SO};
  \definecolor{strokecolor}{rgb}{0.2,0.2,0.2};
  \node (SAT) at (794.0bp,316.0bp) [draw=strokecolor,rectangle,rounded,filled,karp] {SAT};
  \definecolor{strokecolor}{rgb}{0.2,0.2,0.2};
  \node (ThreeSAT) at (507.0bp,260.0bp) [draw=strokecolor,rectangle,rounded,filled,karp] {3SAT};
  \definecolor{strokecolor}{rgb}{0.2,0.2,0.2};
  \node (Clique) at (583.0bp,260.0bp) [draw=strokecolor,rectangle,rounded,filled,karp] {CLIQUE};
  \definecolor{strokecolor}{rgb}{0.2,0.2,0.2};
  \node (ThreeDimMatching) at (700.0bp,260.0bp) [draw=strokecolor,rectangle,rounded,filled,karp] {\shortstack{3-DIM\\MATCHING}};
  \definecolor{strokecolor}{rgb}{0.33,0.33,0.33};
  \node (NTMAccept) at (794.0bp,260.0bp) [draw=strokecolor,rectangle,rounded,filled] {\shortstack{NTM\\ACCEPTANCE}};
  \definecolor{strokecolor}{rgb}{0.33,0.33,0.33};
  \node (NAESAT) at (908.0bp,260.0bp) [draw=strokecolor,rectangle,rounded,filled] {NAE-SAT};
  \definecolor{strokecolor}{rgb}{0.33,0.33,0.33};
  \node (ThreeCol) at (1086.0bp,260.0bp) [draw=strokecolor,rectangle,rounded,filled] {3-COLORABILITY};
  \definecolor{strokecolor}{rgb}{0.33,0.33,0.33};
  \node (OneInSAT) at (273.0bp,200.0bp) [draw=strokecolor,rectangle,rounded,filled] {1-IN-SAT};
  \definecolor{strokecolor}{rgb}{0.2,0.2,0.2};
  \node (VertexCover) at (511.0bp,200.0bp) [draw=strokecolor,rectangle,rounded,filled,karp] {\shortstack{VERTEX\\COVER}};
  \definecolor{strokecolor}{rgb}{0.33,0.33,0.33};
  \node (IndependentSet) at (759.0bp,140.0bp) [draw=strokecolor,rectangle,rounded,filled] {\shortstack{INDEPENDENT\\SET}};
  \definecolor{strokecolor}{rgb}{0.33,0.33,0.33};
  \node (SubgraphIso) at (669.0bp,200.0bp) [draw=strokecolor,rectangle,rounded,filled] {\shortstack{SUBGRAPH\\ISOMORPHISM}};
  \definecolor{strokecolor}{rgb}{0.2,0.2,0.2};
  \node (SetCover) at (233.0bp,140.0bp) [draw=strokecolor,rectangle,rounded,filled,karp] {SET COVER};
  \definecolor{strokecolor}{rgb}{0.2,0.2,0.2};
  \node (HittingSet) at (136.0bp,80.0bp) [draw=strokecolor,rectangle,rounded,filled,karp] {HITTING SET};
  \definecolor{strokecolor}{rgb}{0.2,0.2,0.2};
  \node (FeedbackVertexSet) at (333.0bp,140.0bp) [draw=strokecolor,rectangle,rounded,filled,karp] {\shortstack{FEEDBACK\\VERTEX SET}};
  \definecolor{strokecolor}{rgb}{0.2,0.2,0.2};
  \node (FeedbackArcSet) at (413.0bp,80.0bp) [draw=strokecolor,rectangle,rounded,filled,karp] {\shortstack{FEEDBACK\\ARC SET}};
  \definecolor{strokecolor}{rgb}{0.2,0.2,0.2};
  \node (HamCircuit) at (470.0bp,140.0bp) [draw=strokecolor,rectangle,rounded,filled,karp] {\shortstack{HAMILTON\\CIRCUIT}};
  \definecolor{strokecolor}{rgb}{0.2,0.2,0.2};
  \node (SteinerTree) at (552.0bp,140.0bp) [draw=strokecolor,rectangle,rounded,filled,karp] {\shortstack{STEINER\\TREE}};
  \definecolor{strokecolor}{rgb}{0.33,0.33,0.33};
  \node (EdgeSteinerTree) at (649.0bp,140.0bp) [draw=strokecolor,rectangle,rounded,filled] {\shortstack{EDGE-WEIGHTED\\STEINER TREE}};
  \definecolor{strokecolor}{rgb}{0.2,0.2,0.2};
  \node (SetPacking) at (759.0bp,80.0bp) [draw=strokecolor,rectangle,rounded,filled,karp] {SET PACKING};
  \definecolor{strokecolor}{rgb}{0.33,0.33,0.33};
  \node (DominatingSet) at (233.0bp,80.0bp) [draw=strokecolor,rectangle,rounded,filled] {\shortstack{DOMINATING\\SET}};
  \definecolor{strokecolor}{rgb}{0.33,0.33,0.33};
  \node (GraphCrawling) at (326.0bp,80.0bp) [draw=strokecolor,rectangle,rounded,filled] {\shortstack{GRAPH\\CRAWLING}};
  \definecolor{strokecolor}{rgb}{0.2,0.2,0.2};
  \node (ExactCover) at (68.0bp,140.0bp) [draw=strokecolor,rectangle,rounded,filled,karp] {EXACT COVER};
  \definecolor{strokecolor}{rgb}{0.2,0.2,0.2};
  \node (Knapsack) at (44.0bp,80.0bp) [draw=strokecolor,rectangle,rounded,filled,karp] {KNAPSACK};
  \definecolor{strokecolor}{rgb}{0.2,0.2,0.2};
  \node (ChromaticNumber) at (1166.0bp,200.0bp) [draw=strokecolor,rectangle,rounded,filled,karp] {\shortstack{CHROMATIC\\NUMBER}};
  \definecolor{strokecolor}{rgb}{0.2,0.2,0.2};
  \node (CliqueCover) at (1166.0bp,140.0bp) [draw=strokecolor,rectangle,rounded,filled,karp] {\shortstack{CLIQUE\\COVER}};
  \definecolor{strokecolor}{rgb}{0.2,0.2,0.2};
  \node (DirHamCircuit) at (521.0bp,80.0bp) [draw=strokecolor,rectangle,rounded,filled,karp] {\shortstack{DIRECTED\\HAMILTON CIRCUIT}};
  \definecolor{strokecolor}{rgb}{0.2,0.2,0.2};
  \node (MaxCut) at (880.0bp,140.0bp) [draw=strokecolor,rectangle,rounded,filled,karp] {MAX CUT};
  \definecolor{strokecolor}{rgb}{0.2,0.2,0.2};
  \node (JobSequencing) at (969.0bp,140.0bp) [draw=strokecolor,rectangle,rounded,filled,karp] {\shortstack{JOB\\SEQUENCING}};
  \definecolor{strokecolor}{rgb}{0.2,0.2,0.2};
  \node (Partition) at (992.0bp,200.0bp) [draw=strokecolor,rectangle,rounded,filled,karp] {PARTITION};
  \definecolor{strokecolor}{rgb}{0.33,0.33,0.33};
  \node (ATMAccept 1 true) at (794.0bp,200.0bp) [draw=strokecolor,rectangle,rounded,filled] {\shortstack{ATM\\ACCEPTANCE, 1 BLOCK}};
  \definecolor{strokecolor}{rgb}{0.33,0.33,0.33};
  \node (CQContainment) at (1262.0bp,140.0bp) [draw=strokecolor,rectangle,rounded,filled] {\shortstack{CQ\\CONTAINMENT}};
  \definecolor{strokecolor}{rgb}{0.33,0.33,0.33};
  \node (CQEval) at (1262.0bp,200.0bp) [draw=strokecolor,rectangle,rounded,filled] {\shortstack{CQ\\EVALUATION}};
  \definecolor{strokecolor}{rgb}{0.33,0.33,0.33};
  \node (NAE3SAT) at (908.0bp,200.0bp) [draw=strokecolor,rectangle,rounded,filled] {NAE-3SAT};
  \definecolor{strokecolor}{rgb}{0.33,0.33,0.33};
  \node (SetSplitting) at (1077.0bp,200.0bp) [draw=strokecolor,rectangle,rounded,filled] {\shortstack{SET\\SPLITTING}};
  \definecolor{strokecolor}{rgb}{0.13,0.29,0.53};
  \draw [strokecolor,->,thick] (ESO) ..controls (794.0bp,350.92bp) and (794.0bp,341.61bp)  .. (SAT);
  \definecolor{strokecolor}{rgb}{0.13,0.29,0.53};
  \draw [strokecolor,->,thick] (SAT) ..controls (718.48bp,307.79bp) and (617.06bp,294.89bp)  .. (534.0bp,274.0bp) .. controls (531.97bp,273.49bp) and (529.9bp,272.92bp)  .. (ThreeSAT);
  \definecolor{strokecolor}{rgb}{0.13,0.29,0.53};
  \draw [strokecolor,->,thick] (SAT) ..controls (728.55bp,298.25bp) and (658.69bp,280.37bp)  .. (Clique);
  \definecolor{strokecolor}{rgb}{0.13,0.29,0.53};
  \draw [strokecolor,->,thick] (SAT) ..controls (764.64bp,298.14bp) and (745.13bp,286.93bp)  .. (ThreeDimMatching);
  \definecolor{strokecolor}{rgb}{0.13,0.29,0.53};
  \draw [strokecolor,->,thick] (SAT) ..controls (785.92bp,298.86bp) and (785.39bp,289.55bp)  .. (NTMAccept);
  \definecolor{strokecolor}{rgb}{0.13,0.29,0.53};
  \draw [strokecolor,->,thick] (SAT) ..controls (832.07bp,296.97bp) and (861.33bp,283.11bp)  .. (NAESAT);
  \definecolor{strokecolor}{rgb}{0.13,0.29,0.53};
  \draw [strokecolor,->,thick] (SAT) ..controls (868.88bp,299.52bp) and (967.74bp,281.18bp)  .. (ThreeCol);
  \definecolor{strokecolor}{rgb}{0.1,0.1,0.1};
  \draw [strokecolor,->,thick] (ThreeSAT) ..controls (541.38bp,269.75bp) and (548.97bp,272.23bp)  .. (556.0bp,274.0bp) .. controls (627.59bp,292.01bp) and (712.8bp,304.07bp)  .. (SAT);
  \definecolor{strokecolor}{rgb}{0.13,0.29,0.53};
  \draw [strokecolor,->,thick] (ThreeSAT) ..controls (436.81bp,241.6bp) and (353.74bp,221.01bp)  .. (OneInSAT);
  \definecolor{strokecolor}{rgb}{0.1,0.1,0.1};
  \draw [strokecolor,->,thick] (Clique) ..controls (553.29bp,241.72bp) and (537.45bp,229.37bp)  .. (VertexCover);
  \definecolor{strokecolor}{rgb}{0.1,0.1,0.1};
  \draw [strokecolor,->,thick] (Clique) ..controls (577.17bp,234.59bp) and (586.26bp,203.35bp)  .. (606.0bp,186.0bp) .. controls (613.91bp,179.05bp) and (669.27bp,162.72bp)  .. (IndependentSet);
  \definecolor{strokecolor}{rgb}{0.1,0.1,0.1};
  \draw [strokecolor,->,thick] (Clique) ..controls (609.03bp,241.44bp) and (628.19bp,228.53bp)  .. (SubgraphIso);
  \definecolor{strokecolor}{rgb}{0.1,0.1,0.1};
  \draw [strokecolor,->,thick] (VertexCover) ..controls (547.3bp,223.31bp) and (562.66bp,235.64bp)  .. (Clique);
  \definecolor{strokecolor}{rgb}{0.1,0.1,0.1};
  \draw [strokecolor,->,thick] (VertexCover) ..controls (441.56bp,186.03bp) and (357.16bp,169.84bp)  .. (286.0bp,154.0bp) .. controls (281.75bp,153.05bp) and (277.32bp,152.03bp)  .. (SetCover);
  \definecolor{strokecolor}{rgb}{0.1,0.1,0.1};
  \draw [strokecolor,->,thick] (VertexCover) ..controls (415.25bp,194.72bp) and (238.6bp,183.79bp)  .. (189.0bp,154.0bp) .. controls (166.8bp,140.67bp) and (151.16bp,114.1bp)  .. (HittingSet);
  \definecolor{strokecolor}{rgb}{0.1,0.1,0.1};
  \draw [strokecolor,->,thick] (VertexCover) ..controls (455.18bp,180.81bp) and (409.23bp,165.84bp)  .. (FeedbackVertexSet);
  \definecolor{strokecolor}{rgb}{0.1,0.1,0.1};
  \draw [strokecolor,->,thick] (VertexCover) ..controls (464.59bp,184.91bp) and (439.97bp,173.16bp)  .. (426.0bp,154.0bp) .. controls (414.92bp,138.8bp) and (412.25bp,117.18bp)  .. (FeedbackArcSet);
  \definecolor{strokecolor}{rgb}{0.64,0.0,0.0};
  \draw [strokecolor,->,thick] (VertexCover) ..controls (496.35bp,178.27bp) and (489.54bp,168.64bp)  .. (HamCircuit);
  \definecolor{strokecolor}{rgb}{0.13,0.29,0.53};
  \draw [strokecolor,->,thick] (VertexCover) ..controls (525.65bp,178.27bp) and (532.46bp,168.64bp)  .. (SteinerTree);
  \definecolor{strokecolor}{rgb}{0.13,0.29,0.53};
  \draw [strokecolor,->,thick] (VertexCover) ..controls (559.14bp,178.77bp) and (588.18bp,166.56bp)  .. (EdgeSteinerTree);
  \definecolor{strokecolor}{rgb}{0.1,0.1,0.1};
  \draw [strokecolor,->,thick] (VertexCover) ..controls (540.25bp,186.96bp) and (542.15bp,186.47bp)  .. (544.0bp,186.0bp) .. controls (610.93bp,169.09bp) and (628.72bp,169.49bp)  .. (696.0bp,154.0bp) .. controls (700.93bp,152.87bp) and (706.1bp,151.63bp)  .. (IndependentSet);
  \definecolor{strokecolor}{rgb}{0.1,0.1,0.1};
  \draw [strokecolor,->,thick] (SetCover) ..controls (193.24bp,120.37bp) and (167.58bp,105.21bp)  .. (HittingSet);
  \definecolor{strokecolor}{rgb}{0.1,0.1,0.1};
  \draw [strokecolor,->,thick] (SetCover) ..controls (233.0bp,122.32bp) and (233.0bp,111.15bp)  .. (DominatingSet);
  \definecolor{strokecolor}{rgb}{0.13,0.29,0.53};
  \draw [strokecolor,->,thick] (SetCover) ..controls (261.27bp,121.37bp) and (282.23bp,108.3bp)  .. (GraphCrawling);
  \definecolor{strokecolor}{rgb}{0.1,0.1,0.1};
  \draw [strokecolor,->,thick] (HittingSet) ..controls (176.07bp,99.803bp) and (201.72bp,114.98bp)  .. (SetCover);
  \definecolor{strokecolor}{rgb}{0.13,0.29,0.53};
  \draw [strokecolor,->,thick] (ExactCover) ..controls (60.573bp,121.05bp) and (54.893bp,107.32bp)  .. (Knapsack);
  \definecolor{strokecolor}{rgb}{0.1,0.1,0.1};
  \draw [strokecolor,->,thick] (ChromaticNumber) ..controls (1157.7bp,178.57bp) and (1157.4bp,169.39bp)  .. (CliqueCover);
  \definecolor{strokecolor}{rgb}{0.1,0.1,0.1};
  \draw [strokecolor,->,thick] (CliqueCover) ..controls (1174.3bp,161.37bp) and (1174.6bp,170.55bp)  .. (ChromaticNumber);
  \definecolor{strokecolor}{rgb}{0.1,0.1,0.1};
  \draw [strokecolor,->,thick] (FeedbackVertexSet) ..controls (362.4bp,117.68bp) and (376.98bp,107.11bp)  .. (FeedbackArcSet);
  \definecolor{strokecolor}{rgb}{0.1,0.1,0.1};
  \draw [strokecolor,->,thick] (HamCircuit) ..controls (488.35bp,118.13bp) and (497.03bp,108.26bp)  .. (DirHamCircuit);
  \definecolor{strokecolor}{rgb}{0.13,0.29,0.53};
  \draw [strokecolor,->,thick] (Knapsack) ..controls (44.0bp,61.706bp) and (44.0bp,49.097bp)  .. (ZeroOneIP);
  \definecolor{strokecolor}{rgb}{0.13,0.29,0.53};
  \draw [strokecolor,->,thick] (NTMAccept) ..controls (802.41bp,281.44bp) and (802.58bp,290.59bp)  .. (SAT);
  \definecolor{strokecolor}{rgb}{0.1,0.1,0.1};
  \draw [strokecolor,->,thick] (NTMAccept) ..controls (785.72bp,238.57bp) and (785.43bp,229.39bp)  .. (ATMAccept 1 true);
  \definecolor{strokecolor}{rgb}{0.1,0.1,0.1};
  \draw [strokecolor,->,thick] (ATMAccept 1 true) ..controls (802.27bp,221.37bp) and (802.57bp,230.55bp)  .. (NTMAccept);
  \definecolor{strokecolor}{rgb}{0.1,0.1,0.1};
  \draw [strokecolor,->,thick] (CQContainment) ..controls (1270.3bp,161.37bp) and (1270.6bp,170.55bp)  .. (CQEval);
  \definecolor{strokecolor}{rgb}{0.1,0.1,0.1};
  \draw [strokecolor,->,thick] (CQEval) ..controls (1253.7bp,178.57bp) and (1253.4bp,169.39bp)  .. (CQContainment);
  \definecolor{strokecolor}{rgb}{0.1,0.1,0.1};
  \draw [strokecolor,->,thick] (IndependentSet) ..controls (684.06bp,164.87bp) and (635.38bp,179.51bp)  .. (628.0bp,186.0bp) .. controls (610.72bp,201.18bp) and (601.61bp,226.99bp)  .. (Clique);
  \definecolor{strokecolor}{rgb}{0.1,0.1,0.1};
  \draw [strokecolor,->,thick] (IndependentSet) ..controls (718.18bp,153.96bp) and (718.09bp,153.98bp)  .. (718.0bp,154.0bp) .. controls (650.72bp,169.49bp) and (632.93bp,169.09bp)  .. (566.0bp,186.0bp) .. controls (559.28bp,187.7bp) and (552.05bp,189.74bp)  .. (VertexCover);
  \definecolor{strokecolor}{rgb}{0.1,0.1,0.1};
  \draw [strokecolor,->,thick] (IndependentSet) ..controls (759.0bp,117.46bp) and (759.0bp,106.55bp)  .. (SetPacking);
  \definecolor{strokecolor}{rgb}{0.13,0.29,0.53};
  \draw [strokecolor,->,thick] (NAE3SAT) ..controls (899.34bp,181.05bp) and (892.71bp,167.32bp)  .. (MaxCut);
  \definecolor{strokecolor}{rgb}{0.13,0.29,0.53};
  \draw [strokecolor,->,thick] (NAE3SAT) ..controls (926.17bp,181.72bp) and (939.16bp,169.37bp)  .. (JobSequencing);
  \definecolor{strokecolor}{rgb}{0.1,0.1,0.1};
  \draw [strokecolor,->,thick] (NAE3SAT) ..controls (916.41bp,218.95bp) and (916.83bp,232.34bp)  .. (NAESAT);
  \definecolor{strokecolor}{rgb}{0.13,0.29,0.53};
  \draw [strokecolor,->,thick] (NAESAT) ..controls (934.97bp,240.37bp) and (956.94bp,225.21bp)  .. (Partition);
  \definecolor{strokecolor}{rgb}{0.13,0.29,0.53};
  \draw [strokecolor,->,thick] (NAESAT) ..controls (899.61bp,241.22bp) and (899.17bp,227.85bp)  .. (NAE3SAT);
  \definecolor{strokecolor}{rgb}{0.1,0.1,0.1};
  \draw [strokecolor,->,thick] (NAESAT) ..controls (962.46bp,240.31bp) and (1007.1bp,225.0bp)  .. (SetSplitting);
  \definecolor{strokecolor}{rgb}{0.1,0.1,0.1};
  \draw [strokecolor,->,thick] (OneInSAT) ..controls (210.15bp,181.22bp) and (147.49bp,163.49bp)  .. (ExactCover);
  \definecolor{strokecolor}{rgb}{0.1,0.1,0.1};
  \draw [strokecolor,->,thick] (ThreeCol) ..controls (985.2bp,281.35bp) and (881.63bp,300.43bp)  .. (SAT);
  \definecolor{strokecolor}{rgb}{0.13,0.29,0.53};
  \draw [strokecolor,->,thick] (ThreeCol) ..controls (1110.1bp,241.52bp) and (1127.7bp,228.75bp)  .. (ChromaticNumber);
  \definecolor{strokecolor}{rgb}{0.1,0.1,0.1};
  \draw [strokecolor,->,thick] (ThreeCol) ..controls (1141.2bp,240.81bp) and (1184.4bp,226.56bp)  .. (CQEval);
  \definecolor{strokecolor}{rgb}{0.1,0.1,0.1};
  \draw [strokecolor,->,solid,thick] (la0) ..controls (439.38bp,17.0bp) and (444.36bp,17.0bp)  .. (lt0);
  \definecolor{strokecolor}{rgb}{0.13,0.29,0.53};
  \draw [strokecolor,->,solid,thick] (la1) ..controls (645.71bp,17.0bp) and (650.98bp,17.0bp)  .. (lt1);
  \definecolor{strokecolor}{rgb}{0.64,0.0,0.0};
  \draw [strokecolor,->,solid,thick] (la2) ..controls (871.63bp,17.0bp) and (876.76bp,17.0bp)  .. (lt2);
%
\end{tikzpicture}

